Autonomous drone cinematographer: Using artistic principles to create smooth, safe, occlusion-free trajectories for aerial filming

Autonomous aerial cinematography has the potential to enable automatic capture of aesthetically pleasing videos without requiring human intervention, empowering individuals with the capability of high-end film studios. Current approaches either only handle off-line trajectory generation, or offer strategies that reason over short time horizons and simplistic representations for obstacles, which result in jerky movement and low real-life applicability. In this work we develop a method for aerial filming that is able to trade off shot smoothness, occlusion, and cinematography guidelines in a principled manner, even under noisy actor predictions. We present a novel algorithm for real-time covariant gradient descent that we use to efficiently find the desired trajectories by optimizing a set of cost functions. Experimental results show that our approach creates attractive shots, avoiding obstacles and occlusion 65 times over 1.25 hours of flight time, re-planning at 5 Hz with a 10 s time horizon. We robustly film human actors, cars and bicycles performing different motion among obstacles, using various shot types.

==> inputs_cr/1_intro.tex <==
% !TEX root = ../main.tex

\section{Introduction}
\label{sec:intro}
\vspace{-7mm}

Aerial vehicles are revolutionizing the way both professional and amateur film makers capture shots of actors and landscapes, increasing the flexibility of narrative elements and allowing the composition of aerial viewpoints which are not feasible using traditional devices such as hand-held cameras and dollies. 
% Flying cameras empower individuals with the capability of high-end film studios, permitting people to film scenes that were too expensive or impractical before. 
However, the use of drones for filming today is still extremely difficult due to several motion planning and human-computer interaction challenges. Aerial cinematography incorporates objectives from different areas, such as high-speed flight 
% \citep{mohta2018fast,barry2018high}
\citep{barry2018high}
,inspection and exploration, formation flight \citep{turpin2012trajectory}, and artistic intent \citep{arijon1976grammar,bowen2013grammar}.

% Aerial cinematography incorporates objectives from different robotics areas. Similarly to high-speed flight \citep{mohta2018fast,barry2018high}, the vehicle must generate smooth and safe trajectories, avoiding obstacles in real time. Following literature in inspection and exploration, filming requires reasoning about the location of view points. We can also trace a parallel between cinematography and formation flight \citep{turpin2012trajectory}, since temporal reasoning plays a major role when following a target. In addition, cinematography needs to consider artistic intent \citep{arijon1976grammar} to shape the resulting trajectory, using guidelines such as the rule of thirds, scale and angles with respect to the actors \citep{bowen2013grammar}.

% . A composition of shots
% , which are the smallest unit of photographic coverage of an actor ,
% plays specific roles in the narrative , and each shot is constructed using canonical cinematography .

% There have been several advancements from both industry and researchers in the area of quadrotor filming. Platforms such as the DJI Spark, DJI Phantom and 3DR Solo and can operate in \textit{Follow Mode}, keeping the subject in sight in the middle of the camera using either a GPS or appearance tracker \citep{joubert2016towards}. However, such maneuvers are very simplistic in composition, do not avoid obstacles, and require user input for drone height and actor scale adjustment. A recent product, Skydio's R1 drone \citep{skydio2018} seems to get closer to addressing most objectives of aerial cinematography by planning safe trajectories over a prediction of the actor's motion \rbnote{what else should I say about skydio? I feel that it's important}. In academia, \citet{joubert2016towards} proposed a method to interpolate between two shots without colliding with the actors, while Nageli et al.~\citep{nageli2017real,nageli2017real2} used a model-predictive-control (MPC) method to generate time-dependent trajectories and \citet{coaguila2016selecting} used a PD control to move the drone towards the a desired position. However, these approaches only work with low-complexity shots, with static or low-speed actors in highly controlled environments with either motion-capture systems or RTK GPS, and they do not address obstacle avoidance at all or in the case of \citet{nageli2017real} cannot deal with arbitrary obstacle shapes, only ellipsoidal objects. \rbnote{am I attacking them too much?}

% Our key insight in this work is that this problem can be efficiently solved as a smooth trajectory optimization, treating quadrotor and camera motion independently. We propose a novel differentiable objective function that measures the occlusion and shot quality of viewpoints in the drone trajectory. Since trajectory smoothness is critical, we employ a covariant gradient descent~\citep{ratliff2009chomp} that only perturbs the trajectory along a smooth Riemannian manifold. This descent rule not only preserves smoothness at each iteration but quickly converges to a local optima by dispersing gradients across the trajectory. As for the camera, we assume it is mounted on a gimbal with independent movement, and we use a tracker to place the actor at the correct screen position purely based on the image stream. 

Previous approaches in aerial filming do not address the complete problem in a sufficiently generalizable manner to be used in real-life scenarios. Off-line trajectory generation cannot be used for most practical situations, and the on-line trajectory generation methods that have been proposed have limitations such as ignoring artistic objectives or only dealing with limited obstacle representations (ignoring obstacles altogether in many cases).

Our key insight in this work is that this problem can be efficiently solved in real-time as a smooth trajectory optimization. 
% This method allows us to plan fast, obtaining safe trajectories in arbitrary world representations, following cinematography guidelines. 
Our contributions in this paper are threefold: (1) we formalize the aerial filming problem following cinematography guidelines for arbitrary types of shots and arbitrary obstacle shapes, (2) we present an efficient optimization method that exploits covariant gradients of the objective function for fast convergence, and (3) for over 1.25 hours of flight time while re-planning, we experimentally show robustness in real-world conditions with different types of shots and shot transitions, actor motions, and obstacle shapes. The supplementary video shows examples of trajectories: \small{\url{https://youtu.be/QX73nBBwd28}}\normalsize.

% To the best of our knowledge this is the first paper to present a generalizable framework for generating smooth, safe, occlusion-free trajectories in real-world conditions based on generic shot configurations, permitting shot transitions, running in real time and validated in real-world experiments.

==> inputs_cr/2_prob_related.tex <==
% !TEX root = ../main.tex
\vspace{-5mm}
\section{Problem definition and related work}
\label{sec:related_work}
\vspace{-7mm}

\begin{figure}[t]
    \center
    \includegraphics[scale=.36]{figs/cover_pic_blocks}
    \caption{Side shot of a person filmed by the drone cinematographer: a) Time-lapse of actor and drone. b) Trajectory generation, where the actor's motion forecast is in purple, the desired cinematography position is in blue, and the optimized trajectory is shown in red. c) Resulting drone camera image}
    \label{fig:cover_pic_blocks}
\end{figure}

Following literature in cinematography \citep{arijon1976grammar,bowen2013grammar}, we identified a small set of parameters that can define a large span of shot types (Figure~\ref{fig:cine_params}). We define \textit{static shots} as shots whose parameters remain static over time, independently of the motion of the actor in the environment, and \textit{dynamic shots} as having time-dependant parameters. We focus on scenarios where one quadrotor is filming one actor, with trajectories $\Path{q}$ and $\Path{a}$ respectively, where $\Path{}(t)$ maps time $t\in [0,t_f]$ to a configuration.

% \textit{Shot scale}, $ss$, given in [m/screen height], corresponds to the length in meters that a vertical segment on the camera sensor would have if projected at a distance corresponding to $\abs{p_{quad}-p_{actor}}$. The scale value would be roughly $0.5$, $1.0$ and larger than $5.0$ for close, medium and long shots respectively.

% \textit{Line of action angle}, $\phi_{rel} \in [0,2\pi]$, corresponds to the angle with respect of the $x$ axis of the projection of the vector $v_{actor}^{quad}$ on the $xy$ plane of $B_{actor}$. 

% \textit{Screen position}, $sp_x,sp_y \in [0,1]$, is the desired location of the actor on screen space.

% \textit{Tilt angle}, $\theta_{rel} \in [-\pi,\pi]$, corresponds to the angle with respect from $xy$ plane of $B_{actor}$ of the vector $v_{actor}^{quad}$. 


% \subsection{Configurations, trajectories and costs}
% In addition, we define a trajectory $\Path{}$ as function mapping time $t \in [0,t_f]$ to configurations $c$.  and both have trajectories defined as $\Path{a}$ and $\Path{q}$ respectively. 
In a generic framework for aerial filming, the motion planner's objective is to minimize a cost function $\costFn{\Path{q}}$, that results in a smooth, safe, occlusion-free trajectory that follows our artistic guidelines as closely as possible:
\vspace{-0.0mm}
\small{
\begin{center} 
$\costFn{\Path{q}} = \costFnShot{\Path{q},\Path{a}} + \costFnSmooth{\Path{q}} + \costFnOcc{\Path{q},\Path{a}} + \costFnObs{\Path{q}}$
\end{center}
}
\vspace{-0.0mm}
\normalsize
% that map time to a configuration $\Path{}(t) = c = [p,q]^T$.

% Given that we aim to operate our quadrotor in real-world scenarios without the use of motion-capture systems nor expensive and impractical RTK GPS systems for actor localization \rbnote{too strong of a comment? does that offend prev authors?}, we took an important decision of decoupling the motion of the quadrotor and gimbal in the trajectory. Therefore, we define the quadrotor trajectory only in terms of position and yaw: $\Path{quad}(t) = [p_{quad},\psi_{quad}]^T$. With this approach, even if we receive a noisy actor trajectory $\Path{actor}$ coming from either conventional GPS or a visual estimation system, we can still orient the camera independently of $\Path{quad}$, correcting for localization errors only using the current image stream before we re-plan.

% Decoupling gimbal and quadrotor orientation also benefits finding an ideal cinematography configuration: for a given actor pose, we can now analytically define a configuration $c_{quad} = [p_{quad},\psi_{quad}]^T$ that lies on a sphere with centered at the actor, oriented towards her. The radius is calculated based on the desired shot scale $r = \frac{f}{ss}$, and the polar and azimuth angles are drawn directly from $\phi_{rel}$ and $\theta_{rel}$. Without decoupling, we would have conflicting objectives coming from the desired screen position, which would require solving an optimization problem to obtain the ideal filming configuration.



% In this equation, $\costShot{}$ represents the shot quality, penalizing the shot distance from $\Path{quad}$ to $\Path{shot}$, which would the ideal trajectory solely according to our parameters. $\costSmooth$ is a penalty on the non-smoothness caused by sudden motions and noisy predictions, which harm the resulting footage. $\costOcc$ penalizes an occluded view towards the actor, and $\costObs$ is used for obstacle avoidance. For obstacle avoidance, we assume that we know the configuration of obstacles, static or dynamic, in the environment, and they can have arbitrary shapes. All costs are detailed in Section~\ref{sec:approach}.

This framework borrows concepts from the disparate fields of virtual cinematography, world representation and smooth trajectory generation. 
Camera control in virtual cinematography is typically on through-the-lens control
% ~\cite{christie2008camera,gleicher1992through,drucker1994intelligent,lino2011director}
~\cite{christie2008camera}
but disregards real-world limitations such as robot physics constraints and noisy motion predictions. 
When dealing with arbitrary real-life environments, voxel occupancy maps
% ~\citep{thrun2005probabilistic}
and truncated signed distance field (TSDF)
% ~\citep{newcombe2011kinectfusion,klingensmith2015chisel}
~\citep{newcombe2011kinectfusion}
are common representations, and can supply distance and gradient of a point to nearest object surface. 
% TSDF supplies the distance and gradient of a point to the nearest object surface, what can be exploited by planning approaches.
% When reasoning about viewpoints and the environment, the world is usually represented using voxel occupancy maps~\citep{thrun2005probabilistic} and representations such as the truncated signed distance field (TSDF)~\citep{newcombe2011kinectfusion,klingensmith2015chisel} can be computed on-line and provide a nice abstraction layer for planning approaches, supplying the distance and gradient to nearest object surface. 
Aerial trajectory generation methods~\citep{shim2003decentralized,mellinger2011minimum} are typically designed for aggressive flight and rely on easy to evaluate objective or constraint functions. 
% such model predictive control (MPC)~\citep{shim2003decentralized},
% to exploiting the differential flatness of the dynamics to generate 
% minimum snap trajectories~\citep{mellinger2011minimum}, along with more efficient solvers~\citep{deits2015efficient,liu2017planning} are typically designed for aggressive flight and
% rely on efficient representations of the environment and 
In general domains, we find techniques with more relaxed requirements
% ~\citep{ratliff2009chomp,schulman2013finding,kalakrishnan2011stomp,kobilarov2012cross}
~\citep{ratliff2009chomp,schulman2013finding}
. We build on CHOMP~\citep{ratliff2009learning} due to its simple update rule that is amenable to new cost functions.
% and its speed of convergence due to use of covariant gradients.

% Camera control in virtual cinematography has been extensively examined by the computer graphics community as reviewed by \cite{christie2008camera}. These methods typically reason about the utility of a viewpoint in isolation and employ either optimization based approaches to find good viewpoints or reactive approaches to track the actor. The focus is typically on through-the-lens control where a virtual camera is manipulated while maintaining focus on certain image features~\cite{gleicher1992through,drucker1994intelligent,lino2011director}. However, virtual cinematography is free of several real-world limitations such as robot physics constraints, noise in actor prediction and noisy representations of objects in the world. 

% Dealing with imperfect representations of the world becomes a bottleneck for viewpoint optimization in physical environments. As the world is sensed online, it is usually incrementally mapped using voxel occupancy maps~\citep{thrun2005probabilistic}. To evaluate a viewpoint, methods typically raycast on such maps which can be very expensive~\citep{isler2016information,Charrow-RSS-15}. Recent advances in mapping have led to better representations that can incrementally compute the \emph{truncated signed distance field (TSDF)}~\citep{newcombe2011kinectfusion,klingensmith2015chisel}, i.e. return the distance and gradient to nearest object surface for a query. TSDFs are a nice abstraction layer for planning approaches and has already been used to efficiently compute collision free trajectories for a UAV~\citep{oleynikova2016voxblox}.

% Smooth trajectory generation offers a principled way to holistically reason about the entire sequence of viewpoints, i.e the time spent in occlusion, proximity to obstacles, the overall shot quality and robustness to noisy actor predictions. Methods vary from full fledged model predictive control~\citep{shim2003decentralized} to exploiting the differential flatness of the dynamics to generate minimum snap trajectories~\citep{mellinger2011minimum}. While such optimization problems are non-convex, efficient approximate methods can be derived by decomposing the space into convex regions and applying either SOS programming~\citep{deits2015efficient} or quadratic programming~\citep{liu2017planning}. 
% However, such methods are typically designed for aggressive flight and rely on efficient representations of the environment and easy to evaluate objective or constraint functions. 
% Outside of the domain of UAVs, there are several general trajectory optimization techniques that have relaxed requirements - CHOMP~\citep{ratliff2009chomp} that operates on TSDFs, TrajOpt~\citep{schulman2013finding} that operate on penetration distances, STOMP~\citep{kalakrishnan2011stomp} and CrossEntropy~\citep{kobilarov2012cross} that is completely gradient free. Of these methods, we build on CHOMP due to its simple update rule that is amenable to new cost functions and its speed of convergence due to use of covariant gradients.

% There is substantial recent work on aerial filming from different fronts.
On aerial filming, \citet{roberts2016generating} generate off-line trajectories given infeasible human-defined key-frames and \citet{joubert2015interactive} provide a tool for interactive off-line design of camera trajectories.
\citet{lino2015intuitive} analytically interpolate between viewpoints while maintaining shot quality. \citet{galvane2017automated} used this method to control quadrotors, but only in obstacle-free environments. \citet{galvane2017directing} considered dynamic targets, however they do not address outdoor settings with occlusion and noise. 
Similarly, \citet{joubert2016towards} transition between shots for static actors while not colliding with them, but offer no solution to obstacle and occlusion avoidance.
Closest to our work, \citet{nageli2017real} apply MPC considering occlusion and safety. However, they plan for short time horizons, use simplistic elliptical representations for all obstacles, and use a high-accuracy motion-capture system. It is not clear if the black-box MPC solver that is used is amenable to other obstacle representations and noise in localization.
In contrast, our method works for long time horizons, has a simple unconstrained update rule, operates on TSDFs, has small runtime onboard and can deal with noise in actor motion predictions.

% \rbnote{we can operate in a multi-drone setting: think a little on how to use occlusion cost function to avoid one drone seeing the other. plus we can treat other drones as moving obstacle representations so we avoid crashing: would have to describe this in problem definition}

% \rbnote{can we also adapt the problem to work with multiple actors? probably not the way things are setup now because would have to couple position together with cam orientation in optimization so we can see both at same time}


==> inputs_cr/3_approach.tex <==
% !TEX root = ../main.tex
\vspace{-5mm}
\section{Approach} 
\label{sec:approach}
\vspace{-7mm}

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\textwidth]{figs/cine_params}
    \caption{Shot parameters, adapted from \citet{bowen2013grammar}: a) shot scale $ss$ corresponds to the size of the projection of the actor on the screen; b) line of action angle $\phi_{rel} \in [0,2\pi]$; c) screen position of the actor projection $sp_x,sp_y \in [0,1]$; d) tilt angle $\theta_{rel} \in [-\pi,\pi]$}
    \label{fig:cine_params}
\end{figure}

Unlike previous work that operate either with high-accuracy indoor motion capture systems or precision RTK GPS outdoors, we use only conventional GPS, resulting in high noise for both drone localization and actor motion prediction. Therefore we decided to decouple the motion of the drone and the camera. The camera is mounted on a 3-axis independent gimbal and can place the actor on the correct screen position, solely using the visual input, despite errors in drone position. With camera decoupled, the trajectory to be optimized becomes $\Path{q}(t) = [x_q(t)\; y_q(t)\; z_q(t)]^T$, assuming that the drone's orientation $\psi_q$ points towards the actor at all times.

\textbf{Designing differentiable cost functions for cinematography}\\
We want trajectories which are smooth, safe, occlusion-free and that follow our artistic guidelines as closely as possible. Following the derivation seen in Section 3 of \citet{zucker2013chomp}, we define a parametrization-invariant smoothness cost that can be expressed as a quadratic function, and an obstacle avoidance cost based on a penalization $c$ of the TSDF, for both the environment and the dynamic actor. In addition, we  define two more cost functions specifically for cinematography:

% \textit{Smoothness}:\\
% $\costFnSmooth{\Path{q}} = \int_0^{t_{f}} \sum_{d=0}^{d_{max}} \alpha_n (D^d \Path{quad}(t))^2 dt \approx \frac{1}{2 (n-1)} Tr \left( \sum_{d=1}^{d_{max}} \alpha_d(\xi^T A_d \xi + 2\xi^T b_d + c_d) \right)$\\
% , we choose the smoothness function to be in quadratic form where $A$ and $b$ can be computed using the a discrete differentiation matrix and the boundary conditions. In this work we employ derivatives from $1^{st}$ up to $3^{rd}$ order.

% \textit{Obstacle avoidance}:\\
% $\costFnObs{\Path{q}} = \int_{t=0}^{t_{f}} c_D(\xi(t)) \norm{\frac{d}{dt}\xi(t)}{} dt$\\
% Again following the derivation of \citet{zucker2013chomp}, we assume we have an interface that gives us the TSDF information about the environment in the form of a differentiable function $D: \real^3 \to \real$ that maps a point in the workspace to a truncated signed distance field, and a function $c_D: \real^3 \to \real$ that maps TSDF into a cost: 
% $
% c_D(p) = 
%     \begin{cases}
%       -D(p)+\frac{1}{2} \epsilon_{obs} & D(p)<0\\
%       \frac{1}{2\epsilon_{obs}}(D(p)-\epsilon_{obs}) & 0<D(p)\leq\epsilon_{obs}\\
%       0&\text{otherwise}
%     \end{cases}
% $

\textit{Shot quality}:
\vspace{-0.0mm}
\small{
\begin{center} 
$\costFnShot{\Path{q},\Path{shot}} = \frac{1}{t_{f}} \frac{1}{2} \int_0^{t_{f}} ||\Path{q}(t)-\Path{shot}(t)||^2 dt \approx \frac{1}{2(n-1)} Tr(\Path{q}^T A_{shot} \Path{q} + 2\Path{q}^T b_{shot} + c_{shot})$\\
$\nabla \costFnShot{\Path{q}} = \frac{1}{n-1}(A_{shot}\Path{q}+b_{shot})$ 
\end{center}
}
\vspace{-0.0mm}
\normalsize
Written in a quadratic form, it measures the average squared distance between $\Path{q}$ and an ideal trajectory $\Path{shot}$ that only considers positioning via cinematography parameters. $\Path{shot}$ can be computed analytically: for each point $\Path{a}(t)$ in the actor motion prediction, the drone position lies on a sphere centered at the actor with radius calculated via the shot scale, and angles given by $\phi_{rel}$ and $\theta_{rel}$, as in Figure~\ref{fig:cine_params}.

\textit{Occlusion avoidance}:
\vspace{-0.0mm}
\small{
\begin{center} 
$\costFnOcc{\Path{q},\Path{a}} = \int_{t=0}^{t_{f}} \int_{\tau=0}^{1}\; c(p(\tau)) \norm{\frac{d}{d\tau} p(\tau)}{} d\tau \, \norm{\frac{d}{dt}\Path{q}(t)}{} dt$
\end{center}
}
\vspace{-0.0mm}
\normalsize
% Occlusion means that the camera does not have direct visibility to the actor, which happens if an obstacle is in between them. 
Even though the concept of occlusion is binary, \textit{i.e}, we either have or don't have visibility of the actor, a major contribution of our work is to define a differentiable cost that expresses a viewpoint's occlusion intensity for arbitrary obstacle shapes.
% Formalizing the concept of occlusion cost for arbitrary obstacle shapes is , and has not been addressed in any prior work in the field for generic obstacle shapes.
Mathematically, occlusion is the integral of the TSDF cost $c$ over a 2D manifold connecting both trajectories $\Path{q}$ and $\Path{a}$. We then have the functional gradient:
\vspace{-0.0mm}
\small{
\begin{center} 
$\nabla \costFnOcc{\Path{q},\Path{a}}(t) = \int_{\tau=0}^{1}
\nabla c(p(\tau)) |L| |\dot{q}| \left [ I - (\hat{\dot{q}}+\tau(\frac{\dot{a}}{|\dot{q}|}-\hat{\dot{q}}) ) \hat{\dot{q}}^T \right ]
- c(p(\tau)) |\dot{q}| \left [ \hat{L}^T + \frac{\hat{L}^T \dot{L} \hat{\dot{q}}{}^T}{|\dot{q}|} + |L|\kappa^T \right ]
d\tau$
\end{center}
}
\vspace{-0.0mm}
\normalsize

Where:
\vspace{-0.0mm}
\small{
\begin{center}
$q=\Path{q}(t), \quad a=\Path{a}(t),\quad p(\tau) = (1-\tau)q + \tau a, 
\quad \hat{v} = \frac{v}{|v|},\quad \kappa = \frac{1}{|\dot{q}|^2}(I-\hat{\dot{q}} \hat{\dot{q}}^T) \ddot{q}, \quad L = a-q$
\end{center}
}
\vspace{-0.0mm}
\normalsize

Intuitively, the term $\nabla c(p(\tau))$ is related to variations of the gradient in space, and the term $\tau$ acts as a lever for the gradient. The term $c(p(\tau))$ is linked to changes in path length between camera and actor.

% where $\quad p(\tau) = (1-\tau)\Path{q}(t) + \tau \Path{a}(t)$, $\hat{v} = \frac{v}{\norm{v}{}}$, $\kappa = \frac{1}{\norm{\dot{p_j}}{}^2}(I-\hat{\dot{p_j}} \hat{\dot{p_j}}^T) \ddot{p_j}$, and $L = \Path{a}(t)- \Path{q}(t)$\\

% $\nabla \costFnOcc{\Path{q},\Path{a}} = \sum_{i=1}^{m}\ f_i\ \Delta \tau,\quad \text{with} \quad \Delta \tau = \frac{1}{m-1} \quad \text{and:}\\
%   f_i = \nabla c_D(l(\tau_i))\ |L|\ \norm{\dot{p_j}_{q}}{}\  \left [ I_{2x2} - (\hat{\dot{p_{j}}}{}_{q}+\tau(\frac{\dot{p_j}_{a}}{\norm{\dot{p_j}_{q}}{}}-\hat{\dot{p_{j}}}{}_{q}) ) \hat{\dot{p_{j}}}{}_{q}^T \right ]
%   - c_D(l(\tau_i))\ \norm{\dot{p_j}_{q}}{}\ \left [ \hat{L}^T + \frac{\hat{L}^T L' \hat{\dot{p_{j}}}{}_{q}^T}{\norm{\dot{p_j}_{q}}{}} + |L|\kappa^T \right ]\\
%   \text{and}\quad L = p_j{}_{a}- p_j{}_{q} \quad \kappa = \frac{1}{\norm{\dot{p_j}}{}^2}(I-\hat{\dot{p_j}} \hat{\dot{p_j}}^T) \ddot{p_j}$\\


% $\quad \text{with} \quad \Delta \tau = \frac{1}{m-1} \quad \text{and:}\\
%   f_i = \nabla c_D(l(\tau_i))\ |L|\ \norm{\dot{p_j}_{q}}{}\  \left [ I_{2x2} - (\hat{\dot{p_{j}}}{}_{q}+\tau(\frac{\dot{p_j}_{a}}{\norm{\dot{p_j}_{q}}{}}-\hat{\dot{p_{j}}}{}_{q}) ) \hat{\dot{p_{j}}}{}_{q}^T \right ]
%   - c_D(l(\tau_i))\ \norm{\dot{p_j}_{q}}{}\ \left [ \hat{L}^T + \frac{\hat{L}^T L' \hat{\dot{p_{j}}}{}_{q}^T}{\norm{\dot{p_j}_{q}}{}} + |L|\kappa^T \right ]\\
%   \text{and}\quad L = p_j{}_{a}- p_j{}_{q} \quad \kappa = \frac{1}{\norm{\dot{p_j}}{}^2}(I-\hat{\dot{p_j}} \hat{\dot{p_j}}^T) \ddot{p_j}$

% We can also analytically compute their gradients, and we do so in discretized form without loss of generality. Note that in the following equations $\Path{q}(t_j)=p_j$, and $\hat{v}$ is a normalized vector):\\
% $\nabla \costFnSmooth{\Path{q}} = \frac{1}{(n-1)}(A_{smooth}\xi+b_{smooth})$\\
% $\nabla \costFnObs{\Path{q}(t_j)} = \norm{\dot{p_j}}{} \lparen \; \lparen I - \hat{\dot{p_j}} \hat{\dot{p_j}}^T \rparen \nabla c_D(p_j) -c_D(p_j) \kappa \;\rparen\\
%     \text{where:}\quad \kappa = \frac{1}{\norm{\dot{p_j}}{}^2}(I-\hat{\dot{p_j}} \hat{\dot{p_j}}^T) \ddot{p_j}$\\

% Decoupling gimbal and quadrotor orientation also benefits finding an ideal cinematography configuration: for a given actor pose, we can now analytically define a configuration $c_{quad} = [p_{quad},\psi_{quad}]^T$ that lies on a sphere with centered at the actor, oriented towards her. The radius is calculated based on the desired shot scale $r = \frac{f}{ss}$, and the polar and azimuth angles are drawn directly from $\phi_{rel}$ and $\theta_{rel}$. Without decoupling, we would have conflicting objectives coming from the desired screen position, which would require solving an optimization problem to obtain the ideal filming configuration.

% Here we present the definition of the differentiable cost functions present in the objective $\costFn{\Path{quad}}$, together with the covariant functional gradient descent method used to optimize it. 

% Although the problem is defined in its continuous form, we use a discretized approximation of the trajectories for the solver. In addition, we decouple the trajectory's yaw motion from the position. The yaw of each waypoint is added at the end of the process, with the quadrotor's heading pointing towards the actor at each time step. Therefore, we define our optimization variable with $n-1$ points as: $\Path{quad} =[p_1\;p_2\;...\;p_{n-1}] = [p_{1x}\;p_{1y}\;p_{1z}\;...\;p_{nz}]$, with an additional point $p_0$ being the starting point of the trajectory, defining the boundary conditions.

% \subsection{Designing differentiable cost functions for cinematography}
% The functional $\costFn{\Path{quad}}$ is defined for continuous functions, but here we also present the discretized versions.

% \textbf{Shot quality}
% Shot quality measures the distance between $\Path{quad}$ and the ideal trajectory according solely to the cinematography parameters, $\Path{shot}$, and can be written as a quadratic cost:

% \begin{align}
%     &\costFnShot{\Path{quad}} = \frac{1}{\int_0^{t_{final}} dt} \frac{1}{2} \int_0^{t_{final}} ||p_{t}-p_{t\ shot}||^2 dt\\
%     &\costFnShot{\Path{quad}} = \frac{1}{(n-1)} \frac{1}{2} \sum_{t=1}^{n} ||p_{t}-p_{t\ shot}||^2\\
%     &\costFnShot{\Path{quad}} = \frac{1}{2(n-1)} ||K_{shot}\xi+e||^2 = \frac{1}{2(n-1)} trace(\xi^T A_{shot} \xi + 2\xi^T b_{shot} + c_{shot})\\
%     &\nabla \costFnShot{\Path{quad}} = \frac{1}{n-1}(A_{shot}\xi+b_{shot})
% \end{align}

% Where $K_{shot} = -I$ and $e_{shot} = \Path{shot}$

% \textbf{Smoothness}
% Following the derivation of \citet{zucker2013chomp}, we choose the smoothness function to be in the quadratic form:

% \begin{align}
%     &\costFnSmooth{\Path{quad}} = \int_0^{t_{final}} \sum_{d=0}^{d_{max}} \alpha_n (D^d \Path{quad}(t))^2 dt\\
%     &\costFnSmooth{\Path{quad}} = \sum_{d=1}^{d_{max}} \alpha_d \frac{1}{(n-1)} \frac{1}{2} \sum_{t=1}^{n} \norm{\frac{p_{t}^d-p_{t-1}^d}{\Delta t}}{}^2\\
%     &\costFnSmooth{\Path{quad}} = \frac{1}{2 (n-1)} Tr \left( \sum_{d=1}^{d_{max}} \alpha_d(\xi^T A_d \xi + 2\xi^T b_d + c_d) \right)\\
%     &\nabla \costFnSmooth{\Path{quad}} = \frac{1}{(n-1)}(A_{smooth}\xi+b_{smooth})
% \end{align}

% Where $A$ and $b$ can be computed using the a discrete differentiation matrix and the boundary conditions. In this work we employ derivatives from $1^{st}$ up to $3^{rd}$ order.

% \textbf{Obstacle avoidance}
% Again following the derivation of \citet{zucker2013chomp}, we assume we have full knowledge of the environment in the form of a differentiable function $D: \real^3 \to \real$ that maps a point in the workspace to a truncated signed distance field (Figure~\ref{fig:obs_and_occ}a). In practice, we have an occupancy grid representation of our environment and an interface that computes the signed distance in a moving grid together with the robot. We also assume a function $c_D: \real^3 \to \real$ of the form:

% \begin{align}
%     &c_D(p) = 
%     \begin{cases}
%       -D(p)+\frac{1}{2} \epsilon_{obs} & D(p)<0\\
%       \frac{1}{2\epsilon_{obs}}(D(p)-\epsilon_{obs}) & 0<D(p)\leq\epsilon_{obs}\\
%       0&\text{otherwise}
%     \end{cases}
% \end{align}

% Now we can define the obstacle avoidance cost and its gradient for a particular point of the trajectory $p_j$ at time $t_j$ (note: $\hat{v}$ denotes a normalized vector):

% \begin{align}
%     &\costFnObs{\Path{quad}} = \int_{t=0}^{1} c_D(\xi(t)) \norm{\frac{d}{dt}\xi(t)}{} dt\\
%     &\nabla \costFnObs{\Path{quad}(t_j)} = \norm{\dot{p_j}}{} \lparen \; \lparen I - \hat{\dot{p_j}} \hat{\dot{p_j}}^T \rparen \nabla c_D(p_j) -c_D(p_j) \kappa \;\rparen\\
%     &\text{where:}\quad \kappa = \frac{1}{\norm{\dot{p_j}}{}^2}(I-\hat{\dot{p_j}} \hat{\dot{p_j}}^T) \ddot{p_j}
% \end{align}

% \begin{figure}[t]
%     \sidecaption
%     \includegraphics[scale=.20]{figs/occ_grad}
%     \caption{Occlusion cost gradient acting over a camera trajectory in a signed distance field. Actor trajectory is shown as crosses.}
%     \label{fig:occ_grad}
% \end{figure}

% \textbf{Occlusion avoidance}
% Occlusion means that the camera does not have direct visibility to the actor, which happens if an obstacle is in between them. Even though the concept of occlusion is binary (we either have or don't have visibility of the actor), during the optimization process we need a gradient to guide the trajectory out of the occlusion zone. Formalizing the concept of occlusion gradient is a major contribution of this work, and has not been addressed in any prior work in the field for generic obstacle shapes. 

% Again, we use the concept of truncated signed distance field. The intuition behind our occlusion cost is that the deeper the ray connecting camera and actor goes into an obstacle, the worse the occlusion for that configuration. If we consider this quantity integrated over the entire $\{\Path{quad},\Path{actor}\}$ pair, it is equivalent of integrating $c_D$ over a plane manifold connecting both trajectories. Mathematically, we define a cost independent of trajectory re-timing: 

% \begin{align}
%   &\costFnOcc{\Path{quad},\Path{actor}} = \int_{t=0}^{t_{final}} \int_{\tau=0}^{1} c_D(p(\tau)) \norm{\frac{d}{d\tau} p(\tau)}{} d\tau \quad \norm{\frac{d}{dt}\Path{quad}(t)}{} dt\\
%   &\text{where}\quad l(\tau) = (1-\tau)\Path{quad}(t) + \tau \Path{actor}(t)
% \end{align}

% Thus, the gradient of this functional in the discrete form becomes, assuming $m$ points between actor and quadrotor:

% \begin{align*}
%   &\nabla \costFnOcc{\Path{quad},\Path{actor}} = \sum_{i=1}^{m}\ f_i\ \Delta \tau,\quad \text{with} \quad \Delta \tau = \frac{1}{m-1} \quad \text{and:}\\
%   &f_i = \nabla c_D(l(\tau_i))\ |L|\ \norm{\dot{p_j}_{quad}}{}\  \left [ I_{2x2} - (\hat{\dot{p_{j}}}{}_{quad}+\tau(\frac{\dot{p_j}_{act}}{\norm{\dot{p_j}_{quad}}{}}-\hat{\dot{p_{j}}}{}_{quad}) ) \hat{\dot{p_{j}}}{}_{quad}^T \right ]\\
%   &- c_D(l(\tau_i))\ \norm{\dot{p_j}_{quad}}{}\ \left [ \hat{L}^T + \frac{\hat{L}^T L' \hat{\dot{p_{j}}}{}_{quad}^T}{\norm{\dot{p_j}_{quad}}{}} + |L|\kappa^T \right ]\\
%   &\text{and}\quad L = p_j{}_{act}- p_j{}_{quad}
% \end{align*}

% We can think of more intuitive interpretations for each part of the gradient. The term $\nabla c(l(\tau_i))$ is related to variations in the gradient in space: will depend on how the obstacle configuration changes over space. We see the term $\tau$, which acts as a lever effect. The term $c(l(\tau_i))$ on the other hand is related to variations in path length between camera and actor.

% \rbnote{how can I cut down these interpretations? not enough space here}
 % \begin{itemize}
   % \item $\nabla c(l(\tau_i))$: Related to variations in the gradient in space: will depend on how the obstacle configuration changes over space. We see the term $\tau$, which acts as a lever effect. 
   % First, assume that $x'_{act}$ and $x'_{cam}$ are equal: since the relative speeds are equal, a change in the gradient at a particular point of the path $p(\tau_i)$ will have the same effect on the integral over the path as a change in any other point. However, if relative speeds are different we have a lever effect (imagine a triangle): the closer a point is to the camera, the smaller its relative variation will be relative to the original path. Therefore, a change in gradient will be amplified by $(1-\tau_i)$
   % \item $c(l(\tau_i))$: related to variations in path length between camera and actor. 
   % Roughly, imagine that if the cost at a particular point remains the same but relative speeds are different, our path length will be shortened or increased, what will result in a change of the integral of cost over the path. The term $\tau$ does not influence this term because it considers that the cost is constant for each point (only length changes).
 % \end{itemize}

\textbf{Covariant gradient and steepest descent method}\\
Our objective is to minimize the functional $\costFn{\Path{q}}$. Following a first-order Taylor expansion around the current iteration $k$ using gradient $g_k$, we have \citep{ratliff2009learning}:
\vspace{-0.0mm}
\small{
\begin{center}
$\Path{q}{}_{k+1} = \Path{q}{}_{k} - \frac{1}{\lambda} M^{-1} g_k$
\end{center}
}
\vspace{-0.0mm}
\normalsize
% $\Path{quad}{}_{k+1} = \argminprob{\Path{q}} \left\{ \costFn{\Path{q}} + g_k^T(\Path{q}-\Path{q}{}_k) + \frac{\lambda}{2} \norm{\Path{q}-\Path{q}{}_k}{M}^2 \right\}\\
%   \implies \Path{q}{}_{k+1} = \Path{q}{}_{k} - \frac{1}{\lambda} M^{-1} g_k$\\
% \begin{align*}
% 	&\Path{quad}{}_{k+1} = \argminprob{\Path{q}} \left\{ \costFn{\Path{q}} + g_k^T(\Path{q}-\Path{q}{}_k) + \frac{\lambda}{2} \norm{\Path{q}-\Path{q}{}_k}{M}^2 \right\}\\
% 	&\implies \Path{q}{}_{k+1} = \Path{q}{}_{k} - \frac{1}{\lambda} M^{-1} g_k
% \end{align*}
This is equivalent to following a direction of steepest descent on the functional cost. Our metric $M$ is composed by the sum of quadratic terms coming form both $\costSmooth$ and $\costShot$: $M = A_{smooth} + A_{shot}$. $M$ can be seen as an approximation of the Hessian.
% In other words, we can say that we approximate the Hessian of the cost by evaluating only at the cost terms which are in fact quadratic. As described in \citet{ratliff2009learning}, this update rule will render smooth updates to our trajectory towards a local minimum of cost.

% \scnote{
% 	A.
% 	Designing differentiable cost functions. (Big section)
% 	i. closeness cost: how do you solve using SQP, (can we call this a better name like shot quality)
% 	ii. smoothness cost: naturally follows because closeness cost depends on actor trajectory which can be noisy
% 	iii. occlusion cost: the main novel contribution

% 	B. Covariant gradient. What is it? Why is it cool (smoothness, speed)? What does it require? \rbnote{covariant gradient is just a way of doing steepest gradient descent on a cost function. in itself, it is no more special than the newton method. the main innovation comes from the design of the smoothness cost function itself, which is on a Riemannian manifold. This means that we are setting costs on the curvature of these trajectory spaces (Einstein used Riemannian manifolds to set curvature constraints for gravitational forces)} \rbnote{so, in the end the metric inverse is going to consider both the smoothness and closeness cost functions, bc it's just like a regular steepest descent optimization method. there's nothing special about it} \rbnote{hessian augmentation}

% 	C. Augmentations to algorithm
% 	i. Adding squared objective to A metric (not sure if this is a Reimannian metric) \rbnote{it's not riemannian, but it doesn't have to be. we're just doing steepest descent}
% 	ii. HAndling boundary constraint? Why? \rbnote{talk about lookahead and tracking point logic, boundary in smoothness} \rbnote{we don't want a fixed end point for our problem like most manipulation probs - so we manually hack the grad of the vel at the last waypoint so it doesn't shrink the traj}
% 	iii. Initialization \rbnote{use current trajectory as initialization for next, and assume linear extension for future times} \rbnote{covariant gradient maps from smooth to smooth, but not necessarely from non-smooth to smooth, so initialization is very important}
% 	iv. Time Parameterization? (again not an important point) \rbnote{each waypointpoint has a particular time associated with it}
% 	\rbnote{V. talk about algorithm details such as convergence criteria? maybe too much detail}
% }

==> inputs_cr/4_results.tex <==
% !TEX root = ../main.tex
\vspace{-5mm}
\section{Experiments} 
\label{sec:experiments}
\vspace{-7mm}
% In this section we detail experiments performed with our method in simulation and field tests.

% \textbf{Simulation experiments}\\
% We validated our algorithm in 2D scenarios. We considered different obstacle settings, actor trajectories, and initializations for the camera trajectory. Figure~\ref{fig:matlab_result} shows some of the optimized trajectories.

% \begin{figure}[t]
%     \sidecaption
%     \includegraphics[scale=0.30]{figs/matlab_result}
%     \caption{Simulation result in for 2D environment. Noisy actor and drone positions are shown as crosses circles respectively. Intermediate steps of the optimization are shown in color scale from blue to green. Plot of the right shows cost decreasing with iterations.}
%     \label{fig:matlab_result}
% \end{figure}

% \textbf{Field experiments}

\begin{figure}[t]
    \sidecaption
    \includegraphics[scale=0.5]{figs/system_new}
    \caption{System architecture. The vision subsystem controls the camera orientation using only the monocular image, independently of the planning subsystem. Planning uses the drone's and actor's current location, and the environment to generate trajectories for the flight controller.}
    \label{fig:system2}
\end{figure}

% Our objective was to test if: (a) our algorithm is robust and fast enough to work on a real life scenario running on an onboard computer, and (b) the occlusion cost function significantly improves the quality of the camera image in comparison with pure obstacle avoidance.
% and (c) specially when noise is present, planning trajectories by minimizing the integral of cost over time renders much smoother trajectories than just reasoning about the current best viewpoint.

Our robot is the  DJI M210 drone and we use the NVIDIA TX2 processor for high-level perception and planning (Figure~\ref{fig:system2}).
% ROS~\citep{ros2018} infrastructure handles node communication. 
In the vision pipeline, we detect the actor using Faster-RCNN~\citep{ren2015faster} with MobileNets \citep{howard2017mobilenets} for feature extraction and Kernelized Correlation Filter (KCF)~\citep{henriques2015high} for tracking, controlling the camera gimbal to keep the actor within the desired screen position. The actor wears a Pixhawk PX4 module on a hat that sends his pose to the onboard computer via radio communication, and a linear Kalman filter estimates his velocity, which is used to predict the actor's pose for the next 10 s. Using a point cloud map of the test site we compute a TSDF map of the region of interest off-line. Re-planning happens at 5 Hz with a 10 s horizon.

\textit{(a) Algorithm robustness:}
We evaluated our algorithm performing different types of static and dynamic shots, following different types of actors: humans, cars and bicycles at different speeds and motion types. In total, we collected over 1.25 hours of flight time while re-planning and avoided obstacles and/or occlusion 65 times. The maximum velocity achieved during the tests was of 7.5 m/s. Figure~\ref{fig:res} summarizes the most representative shots, which are also shown in the supplementary video.

\begin{figure}[t]
    \sidecaption
    \includegraphics[scale=.35]{figs/res_blocks}
    \caption{Results: a) Circling shot around person, b) Side shot following biker, c) Side shot following vehicle. The planned trajectory (red) avoids colliding with and being occluded by the mountain, while remaining smooth even under high actor motion prediction noise. The actor's motion forecast is in purple, and the desired artistic shot is in blue.}
    \label{fig:res}
\end{figure}

\textit{(b) Using occlusion cost function:} For the same shot type, we planned paths with and without the occlusion cost function (Figure~\ref{fig:occlusion_3}).

\begin{figure}[t]
    \sidecaption
    \includegraphics[scale=.24]{figs/occ_comp_blocks}
    \caption{Comparison of planning a) without and b) with occlusion cost function. The occlusion cost function significantly improves the quality of the camera image in comparison with pure obstacle avoidance, for same shot type.}
    \label{fig:occlusion_3}
\end{figure}

\textit{(c) Generating smooth trajectories:} We compare tracking performance under real-world noise between greedily tracking the current artistic viewpoint versus trajectory optimization (Figure~\ref{fig:position_tracking_compare}).
% For the same shot type, we compare our method with a position tracking method that only considers cinematographic parameters.  shows that the position tracking method generates jeryky trajectories that the robot is unable to track well. Instead, our method generates dynamically feasible trajectories that the robot can track well.

\begin{figure}[b]
    \sidecaption
    \includegraphics[scale=.15]{figs/position_tracking_compare}
    \caption{Top-down view of drone motion.
    % comparison between directly tracking the desired artistic viewpoint versus trajectory optimization. 
    For naive tracking of artistic viewpoint the error is high, in the order of meters with respect to the target position, because it ignores dynamic feasibility. In our method the tracking error with respect to the optimized trajectory is small even under real-world noise, because we consider smoothness.}
    \label{fig:position_tracking_compare}
\end{figure}


% \textit{(c) Comparison between position controller and smooth trajectory planning:}\\
% We compared the smoothness of the resulting trajectory from both a position controller and our algorithm. Figure~\ref{fig:smooth_top_view} shows a top view of the resulting trajectories.

% \vspace{-2.5mm}

% \begin{figure}[h]
%     \sidecaption
%     \includegraphics[scale=.20]{figs/smooth_top_view}
%     \caption{Comparison of trajectories from current position controller versus smooth trajectory planning}
%     \label{fig:smooth_top_view}
% \end{figure}

% Robot Platform



% \begin{figure}[t]
%     \center
%     \includegraphics[scale=.40]{figs/performance_plot}
%     \caption{caption}
%     \label{fig:performance_plot}
% \end{figure}

% \begin{figure}[t]
%     \center
%     \includegraphics[scale=.40]{figs/performance_fixed_num_blocks}
%     \caption{caption}
%     \label{fig:performance_fixed_num_blocks}
% \end{figure}

% ii. Comparison to fmincon on a representative dataset \rbnote{idea here is that the covariant gradient speeds up the solution quite a lot}

% \begin{figure}[t]
%     \center
%     \includegraphics[scale=.40]{figs/chomp_vs_fmincon}
%     \caption{caption}
%     \label{fig:chomp_vs_fmincon}
% \end{figure}

% B. Simulation case study \rbnote{vary one axis at a time}
% i. Vary across different environments
% ii. Vary across different actor traj
% iii. Vary across different shots
% iv. Some failure case \rbnote{this should lead the future work discussion}

% \begin{figure}[t]
%     \center
%     \includegraphics[scale=.40]{figs/diff_scenarios}
%     \caption{caption}
%     \label{fig:diff_scenarios}
% \end{figure}


% C. Real experiment 
% i. Planning exp \rbnote{show big table with the types of shots we tried (params), artistic picture of what's hapenning, seq of RVIZ traj and seq of real-life pics -- maybe 1st-person view from rviz as well fused with gimbal pics} \rbnote{talk about params, or is this too technical? talk about avg dist to obstacles during the test?} \rbnote{if we have time, test a baseline approach onyl considering obstacle avoidance but not with occlusion cost fn: video will be bad} \rbnote{should we have metrics such as deviation from original trajectory? dist to obstacles? convergence time of traj? which plots can I make? should I rather do it for sim experiments?} \rbnote{we don't have good footage with spark: add later if we have time}
% \rbnote{ii. just vision experiments -- should we have these? might not have space for all in this paper. maybe save it for a journal paper where we report more extensive results on each part of the system?}

% \begin{figure}[t]
%     \center
%     \includegraphics[scale=.40]{figs/real_life}
%     \caption{caption}
%     \label{fig:real_life}
% \end{figure}

% \begin{figure}[t]
%     \center
%     \includegraphics[scale=.40]{figs/comparison_baselines}
%     \caption{caption}
%     \label{fig:comparison_baselines}
% \end{figure}


==> inputs_cr/5_insights_conclusion.tex <==
% !TEX root = ../main.tex
\vspace{-5mm}
\section{Experimental insights and scheduled experiments}
\label{sec:conclusion}
\vspace{-7mm}
We validated our original hypothesis with the experiments: (a) Our algorithm is robust and fast enough to work on a real life scenario running on an onboard computer, generating safe, smooth, occlusion-free trajectories following artistic guidelines. (b) The occlusion cost function we introduced significantly improves the quality of the resulting image. (c) Planning trajectories renders much less error than naively reasoning about the current best viewpoint.

For the camera-ready version of this paper we want to validate the performance of our algorithm from a statistical perspective, plotting performance curves while varying the complexity of the environment, the actor trajectory, shot type and initialization. In addition, we will study failure cases for the algorithm, and how to avoid them.
% (1) How does the steepest descent algorithm perform in comparison with a standard optimizer? 

% Our approach of composing differentiable objectives has potential impact on information gathering tasks~\citep{arora2017randomized}, agricultural monitoring~\citep{herwitz2004imaging} and visibility planning for safety~\citep{richter2016learning}.

% \rbnote{
% 	Future work:
% 	1. Multi-start chomp: if we were to find the true global opt, a viable approach would be to have multiple starting trajs and optimize all of them to find min cost
% 	2. multi-drone scenario tested in real life
% 	3. multi-actor scenario? does that even make sense with our cost funcs? maybe just have multiple closeness funcs?
% 	3. Gaussian Process CHOMP (Boots et al.), using factor graphs for motion planning to treat trajs as continuous functions rather than discrete waypoints
% }




==> inputs_cr/system.tex <==
% !TEX root = ../main_cr.tex

% \section{Systems and Implementation}
% \label{sec:system}

% \rbnote{join with exp? more details?}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% \rbnote{E. Safety trigger: we stop before hitting things}

% % Robot Platform
% \begin{figure}[t]
%     \center
%     \includegraphics[scale=0.12]{figs/robot-platform}
%     \caption{Robot Platform}
%     \label{fig:robot-platform}
% \end{figure}

% The robot platform we use for experiments shown in Figure~\ref{fig:robot-platform} is based on DJI M210. We use the build-in flight controller in M210 for low level control and the NVIDIA TX2 for high-level perception and planning. The TX2 module contains a quad-core ARM Cortex-A57 processor and a dual-core NVIDIA Denver2 processor, which gives enough processing power to run our trajectory planning, object tracking, and filtering algorithms in real-time. It also contains 256 GPU cores that enable our Covolutional Neural Network (CNN) based object detection module to run at \yfnote{XX} Hz. In addition, 500 GB SSD is added for onboard logging. During the experiments, we use a base station laptop to monitor robot status and send high level commands, such as shot parameters, to the robot. The communication between base station and onboard computer is via Wi-Fi network. To obtain the actor pose, we also mounted a Pixhawk module on a hat weared by the actor. The Pixhawk module will send the actor pose to onboard computer via radio communication. 

% % System Architecture
% \begin{figure}[t]
%     \center
%     \includegraphics[scale=0.2]{figs/system-architecture}
%     \caption{System Architecture}
%     \label{fig:system-architecture}
% \end{figure}

% The system architecture is shown in Figure~\ref{fig:system-architecture}. In the vision pipeline, we detect and track the actor in image space with a monocular camera, then control the camera gimbal to keep the actor within the center region. We adopt Faster-RCNN~\citep{ren2015faster} to detect various types of actors due to its robust performance in terms of detecting small objects. We use MobileNets as the feature extraction network because of its low latency and memory consumption. The detected bounding box becomes the initial ROI to a Kernelized Correlation Filter (KCF)~\citep{henriques2015high} based tracker and the monocular camera image stream will be used to update the tracker. Because of the relative high computation load of using CNN based object detection, we only use Faster-RCNN to detect the actor when the vision pipeline is initialized or KCF based tracking fails. Finally, we use a PD gimbal controller to keep the actor in the center region.

% In the planning pipeline, we estimate the actor motion and plan an optimized trajectory to film the actor based on a set of cinematography parameters. We adopt a linear Kalman filter to estimate the actor velocity and the constant velocity model to predict the actor's motion in a 10 seconds horizon. We use a point cloud map of the test site to compute a signed distance map and a voxel representation of its gradients in space offline. During the test time, we use the pre-computed gradients and M210's build-in state estimation to replan the filming trajectory at 5 Hz.\yfnote{may add more explaination.} The communication between all components uses ROS~\citep{ros2018} infrastructure.

% A detailed runtime and memory usage profiling of major components is shown in Table~\ref{table:runtime}.
% \begin{table}
% 	\begin{center}
% 		\begin{tabular}{ | l | l | l |}
% 		\hline
% 		Module & Runtime (ms) & Memory Usage \\ \hline
% 		Trajectory Optimization & xx & xx \\ \hline
% 		Actor Detection & xx & xx \\ \hline
% 		Actor Tracking & xx & xx \\ \hline 
% 		\end{tabular}
% 		\caption{Runtime and Memory Usage Profiling}
% 		\label{table:runtime}
%     \end{center}
% \end{table}

